Design Information Disclosure under Bidder Heterogeneity in Online Advertising Auctions: Implications of Bid-Adherence Behavior

Bidding is a key element of search advertising, but the variation in bidders' valuations and strategies is often overlooked. Disclosing bid information helps uncover this heterogeneity and enables platforms to tailor their disclosure policies to meet objectives like increasing consumer surplus or platform revenue. We analyzed data from a platform that provided bid recommendations based on historical bids. Our findings reveal that advertisers vary significantly in their strategies: some follow the platform's recommendations, while others create their own bids, deviating from the provided information. This highlights the need for customized information disclosure policies in online ad marketplaces. We developed an equilibrium model for Generalized Second Price (GSP) auctions, showing that adhering to bid recommendations with positive probability is suboptimal. We categorized advertisers as bid-adhering or bid-constructing and developed a structural model for self-bidding to identify private valuations. This model allowed for a counterfactual analysis of the impact of different levels of information disclosure. Both theoretical and empirical results suggest that moderate increases in disclosure improve platform revenue and market efficiency. Understanding bidder diversity is crucial for platforms, which can design more effective disclosure policies to address varying bidder needs and achieve their goals through costless information sharing.

==> reg_group817.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{c}}
\hline\hline
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
            &\multicolumn{1}{c}{bid}&\multicolumn{1}{c}{bid}&\multicolumn{1}{c}{cpc}&\multicolumn{1}{c}{cpc}\\
\hline
T\_t         &       2.193\sym{***}&                     &       0.669\sym{***}&                     \\
            &     (0.394)         &                     &     (0.152)         &                     \\
[1em]
1.group     &                     &       0.256         &                     &     -0.0695         \\
            &                     &     (0.601)         &                     &     (0.243)         \\
[1em]
2.group     &                     &       0.217\sym{*}  &                     &       0.129\sym{***}\\
            &                     &     (0.130)         &                     &    (0.0487)         \\
[1em]
3.group     &                     &           0         &                     &           0         \\
            &                     &         (.)         &                     &         (.)         \\
[1em]
0.T\_t       &                     &           0         &                     &           0         \\
            &                     &         (.)         &                     &         (.)         \\
[1em]
1.T\_t       &                     &       0.633\sym{***}&                     &       0.168\sym{*}  \\
            &                     &     (0.207)         &                     &    (0.0906)         \\
[1em]
0.T\_t#1.group&                     &           0         &                     &           0         \\
            &                     &         (.)         &                     &         (.)         \\
[1em]
0.T\_t#2.group&                     &           0         &                     &           0         \\
            &                     &         (.)         &                     &         (.)         \\
[1em]
0.T\_t#3.group&                     &           0         &                     &           0         \\
            &                     &         (.)         &                     &         (.)         \\
[1em]
1.T\_t#1.group&                     &       5.372\sym{***}&                     &       1.902\sym{***}\\
            &                     &     (1.203)         &                     &     (0.478)         \\
[1em]
1.T\_t#2.group&                     &       1.705\sym{***}&                     &       0.436\sym{***}\\
            &                     &     (0.289)         &                     &    (0.0991)         \\
[1em]
1.T\_t#3.group&                     &           0         &                     &           0         \\
            &                     &         (.)         &                     &         (.)         \\
\hline
\(N\)       &       73044         &       73044         &       73044         &       73044         \\
adj. \(R^{2}\)&       0.903         &       0.908         &       0.866         &       0.868         \\
\hline\hline
\multicolumn{5}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{5}{l}{\footnotesize ad and day fixed effects, cluster at advertiser level}\\
\multicolumn{5}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> sum_table_bid_adhere.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{1}{cccc}}
\hline\hline
            &        mean&          sd&         min&         max\\
\hline
new\_bid     &       22.62&       21.16&        1.00&       99.00\\
s1          &       54.62&       32.46&        2.70&       99.00\\
s2          &       41.87&       26.21&        2.11&       99.00\\
s3          &       33.50&       22.15&        1.00&       99.00\\
\hline
\(N\)       &        3532&            &            &            \\
\hline\hline
\end{tabular}
}


==> temp.tex <==
Figure \ref{fig:adinvestment} displays the discrepancy between the two groups regarding their daily budgets and the average bids they submit. The vertical red line in Figure \ref{fig:adinvestment} represents the beginning of the information release. The red line represents the less sophisticated group's daily average, and the blue line shows the sophisticated group's daily average. The green line represents the daily average bid level in the control city among the top 25th-position advertisers. It is displayed as a control with no information intervention. Before the date of the information release, less sophisticated bidders submitted a similar level of bids and allocated a little higher advertising budget compared to sophisticated bidders. Post-intervention, we observe a significant rise of bids among the less sophisticated group. In contrast, the bid level among the sophisticated group in the treated city and the top bidders in the control city both remain constant. Interestingly, the budget level of the sophisticated group drops over time post-intervention. One reason could be that there is a significant drop in high-budget sophisticated bidders post-intervention, according to Figure \ref{fig:high_drop}. Although we do not have clear evidence on why this group chose to leave, we hypothesize that it might be driven by the fact that this group is worse off post-intervention in their ad performance due to more intense competition on the top ad positions (See figure \ref{fig:ad performance}).


==> temp_figure.tex <==


\begin{figure}[htb!]
\centering
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=.7\linewidth]{naive_sophisticated_budget.png}
  \label{fig:budget}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=.7\linewidth]{naive_sophisticated_avg_bid.png}
  \label{fig:avg_bid}
\end{subfigure}
\caption{Ad Investment}
\footnotesize\textsuperscript{*} Figure \ref{fig:adinvestment} displays the budget and average daily bid for two groups: sophisticated advertisers (shown in blue) and less sophisticated advertisers (shown in red). The green line represents the daily average level in the control city among top 25th-position advertisers. The vertical line reflects the date of information disclosure. 
\label{fig:adinvestment}
\end{figure}

